Light Curves of 213 Type Ia Supernovae from the ESSENCE Survey

The ESSENCE survey discovered 213 Type Ia supernovae at redshifts 0.1 < z < 0.81 between 2002 and 2008. We present their R and I-band photometry, measured from images obtained using the MOSAIC II camera at the CTIO 4 m Blanco telescope, along with rapid-response spectroscopy for each object. We use our spectroscopic follow-up observations to determine an accurate, quantitative classification and a precise redshift. Through an extensive calibration program we have improved the precision of the CTIO Blanco natural photometric system. We use several empirical metrics to measure our internal photometric consistency and our absolute calibration of the survey. We assess the effect of various potential sources of systematic bias on our measured fluxes, and we estimate that the dominant term in the systematic error budget from the photometric calibration on our absolute fluxes is ~1%.

==> MLCS_fitp.tex <==
%\begin{landscape}
\begin{center}
\singlespacing
\scriptsize
%\begin{longtable}{lccccrrrcrcc}
\begin{longtable}{cccccccccccc}
\caption{MLCS2k2 Light-Curve Fit Parameters for ESSENCE \snia\ and ``Ia?'' Objects\label{tab:MLCSfitp}}\\

\hline \hline
ID &
$\mu$\tablenotemark{a} &
$\sigma_{\mu}$ &
$T^{B}_{\text{max}} $ &
$\sigma_{T^{B}_{\text{max}}} $ &
$\Phi_{\text{First}}$\tablenotemark{b} &
$\Phi_{\text{Last}}$ &
$\Delta$ &
$\sigma_{\Delta}$ &
$A_{V}$\tablenotemark{c} &
$\sigma_{A_{V}}$ &
Q\tablenotemark{d} \\
\hline
\endfirsthead

\multicolumn{12}{c}%
{{\bfseries \tablename\ \thetable{} (Continued)}} \\
%{{\bfseries \tablename\ \thetable{} --- continued from previous page}} \\

\hline
ID &
$\mu$\tablenotemark{a} &
$\sigma_{\mu}$ &
$T^{B}_{\text{max}} $ &
$\sigma_{T^{B}_{\text{max}}} $ &
$\Phi_{\text{First}}$\tablenotemark{b} &
$\Phi_{\text{Last}}$ &
$\Delta$ &
$\sigma_{\Delta}$ &
$A_{V}$\tablenotemark{c} &
$\sigma_{A_{V}}$ &
Q\tablenotemark{d} \\
                                                          
\hline
\endhead

\hline \multicolumn{12}{c}{{Continued on next page}} \\ \hline
\endfoot

\hline
\hline
\endlastfoot

b010 & 43.082 & 0.180 & 52592.10 & 1.41   &   -5.626  &   13.912   &  -0.221 & 0.170 &  0.113 & 0.099 & T    \\
b013 & 42.104 & 0.251 & 52586.95 & 1.57   &   -2.646  &   21.850   &  -0.057 & 0.179 &  0.223 & 0.198 & T    \\
b016 & 41.691 & 0.338 & 52583.47 & 1.73   &   -3.361  &   30.618   &  -0.188 & 0.188 &  0.437 & 0.293 & T    \\
b017 & 41.060 & 0.212 & 52594.12 & 0.74   &   -5.632  &   38.048   &  -0.128 & 0.124 &  0.189 & 0.198 & T    \\
b020 & 41.942 & 0.384 & 52600.27 & 0.71   &  -10.604  &    6.934   &  -0.047 & 0.311 &  0.275 & 0.240 & F   \\
b022 & 42.879 & 0.225 & 52595.26 & 1.21   &   -6.619  &    9.742   &  -0.065 & 0.221 &  0.091 & 0.095 & T    \\
c015 & 42.518 & 0.315 & 52617.92 & 0.64   &   -8.658  &   17.846   &  -0.141 & 0.178 &  0.359 & 0.264 & T    \\
d058 & 43.073 & 0.222 & 52941.66 & 1.61   &   -6.037  &   28.048   &  -0.401 & 0.101 &  0.205 & 0.163 & F   \\
d083 & 40.856 & 0.106 & 52936.54 & 0.84   &   -4.045  &   43.207   &  -0.281 & 0.061 &  0.085 & 0.082 & T    \\
d084 & 42.849 & 0.387 & 52936.02 & 1.95   &   -3.202  &    5.324   &  -0.015 & 0.351 &  0.272 & 0.233 & F   \\
d085 & 41.971 & 0.224 & 52941.59 & 0.85   &   -6.815  &   33.086   &  -0.171 & 0.131 &  0.207 & 0.169 & T    \\
d086 & 40.249 & 0.289 & 52945.39 & 0.35   &  -11.111  &   35.450   &  -0.217 & 0.078 &  0.536 & 0.306 & T    \\
d089 & 42.009 & 0.204 & 52929.41 & 2.15   &    1.221  &   25.822   &  -0.108 & 0.148 &  0.184 & 0.162 & T    \\
d093 & 41.779 & 0.135 & 52947.25 & 0.54   &  -11.786  &   40.272   &  -0.265 & 0.079 &  0.095 & 0.100 & T    \\
d097 & 42.226 & 0.143 & 52938.25 & 0.90   &   -4.923  &   40.397   &  -0.227 & 0.082 &  0.113 & 0.109 & T    \\
d099 & 40.515 & 0.230 & 52921.56 & 1.62   &    8.715  &   68.225   &  -0.192 & 0.083 &  0.245 & 0.196 & F   \\
d100 & 38.247 & 0.318 & 52922.91 & 2.02   &    6.997  &   57.974   &  -0.306 & 0.058 &  1.115 & 0.335 & F   \\
d117 & 41.570 & 0.252 & 52948.84 & 0.48   &   -6.691  &   34.923   &   0.231 & 0.190 &  0.240 & 0.191 & T    \\
d149 & 41.498 & 0.255 & 52954.66 & 0.37   &   -9.377  &   33.951   &  -0.100 & 0.091 &  0.306 & 0.214 & T    \\
e108 & 42.370 & 0.140 & 52979.48 & 0.59   &  -11.768  &    9.954   &  -0.338 & 0.111 &  0.097 & 0.102 & T    \\
e132 & 40.765 & 0.265 & 52972.60 & 0.38   &  -10.034  &   25.347   &  -0.139 & 0.105 &  0.513 & 0.275 & T    \\
e136 & 41.796 & 0.264 & 52968.10 & 0.84   &   -5.867  &   23.526   &   0.209 & 0.173 &  0.324 & 0.251 & T    \\
e138 & 43.214 & 0.184 & 52956.30 & 1.10   &   -8.790  &   11.059   &  -0.262 & 0.160 &  0.122 & 0.099 & T    \\
e140 & 43.017 & 0.153 & 52969.00 & 1.81   &   -3.009  &   16.924   &  -0.187 & 0.150 &  0.104 & 0.088 & T    \\
e147 & 43.127 & 0.169 & 52965.73 & 1.86   &   -3.382  &    6.338   &  -0.114 & 0.182 &  0.066 & 0.060 & F   \\
e148 & 42.359 & 0.186 & 52976.14 & 0.60   &   -8.394  &   19.642   &  -0.166 & 0.144 &  0.154 & 0.135 & T    \\
e149 & 42.578 & 0.208 & 52951.74 & 0.71   &  -10.460  &   16.359   &   0.023 & 0.177 &  0.103 & 0.110 & T    \\
f011 & 42.713 & 0.215 & 52985.33 & 1.07   &  -11.207  &    9.637   &   0.079 & 0.204 &  0.121 & 0.115 & T    \\
f041 & 42.910 & 0.128 & 52986.30 & 0.86   &   -9.130  &   10.118   &  -0.289 & 0.123 &  0.077 & 0.077 & T    \\
f096 & 42.031 & 0.355 & 52993.31 & 1.87   &   -3.724  &    7.648   &   0.100 & 0.351 &  0.202 & 0.221 & F   \\
f123 & 42.950 & 0.316 & 52987.52 & 1.07   &   -8.813  &    8.258   &  -0.116 & 0.253 &  0.229 & 0.201 & F   \\
f216 & 43.371 & 0.271 & 52985.39 & 1.46   &   -7.069  &    6.758   &  -0.049 & 0.266 &  0.144 & 0.113 & F   \\
f231 & 43.093 & 0.141 & 52985.81 & 0.84   &   -9.738  &   11.275   &  -0.297 & 0.134 &  0.099 & 0.082 & T    \\
f235 & 41.913 & 0.212 & 52989.61 & 0.70   &  -12.372  &    8.789   &   0.099 & 0.220 &  0.135 & 0.107 & F   \\
f244 & 42.820 & 0.242 & 52984.70 & 2.66   &    0.941  &   11.285   &  -0.076 & 0.250 &  0.164 & 0.137 & T    \\
f301 & 42.864 & 0.390 & 52994.27 & 2.07   &   -5.364  &    2.570   &   0.018 & 0.359 &  0.331 & 0.238 & F   \\
f308 & 42.475 & 0.274 & 52993.72 & 1.14   &   -5.455  &    3.199   &   0.046 & 0.300 &  0.145 & 0.144 & F   \\
g005 & 40.455 & 0.240 & 53293.78 & 0.58   &   -7.185  &   54.406   &  -0.289 & 0.057 &  0.414 & 0.247 & T    \\
g050 & 42.849 & 0.211 & 53301.51 & 1.07   &   -7.785  &   13.430   &  -0.066 & 0.193 &  0.101 & 0.088 & T    \\
g052 & 41.682 & 0.240 & 53297.05 & 0.71   &  -10.122  &   18.795   &   0.320 & 0.194 &  0.169 & 0.171 & T    \\
g055 & 41.127 & 0.327 & 53289.89 & 1.23   &   -5.213  &   40.287   &  -0.142 & 0.138 &  1.278 & 0.310 & T    \\
g097 & 41.698 & 0.275 & 53298.87 & 0.57   &  -11.781  &   38.102   &  -0.386 & 0.075 &  0.292 & 0.253 & T    \\
g120 & 42.273 & 0.228 & 53298.01 & 1.21   &   -7.280  &   17.970   &  -0.046 & 0.180 &  0.204 & 0.156 & T    \\
g133 & 41.890 & 0.221 & 53272.79 & 1.58   &   -4.659  &   57.264   &  -0.230 & 0.144 &  0.180 & 0.156 & T    \\
g142 & 42.164 & 0.376 & 53296.82 & 1.24   &   -6.991  &   20.097   &   0.350 & 0.335 &  0.273 & 0.247 & T    \\
g160 & 42.492 & 0.183 & 53283.51 & 0.96   &  -10.155  &   30.288   &  -0.281 & 0.090 &  0.159 & 0.140 & T    \\
g225 & 43.327 & 0.115 & 53310.91 & 1.12   &  -10.068  &   28.588   &  -0.685 & 0.070 &  0.069 & 0.071 & F   \\
g240 & 43.126 & 0.170 & 53305.94 & 1.26   &   -8.841  &   11.306   &  -0.202 & 0.162 &  0.066 & 0.055 & T    \\
h283 & 42.915 & 0.209 & 53320.54 & 1.56   &   -3.626  &   19.799   &  -0.210 & 0.156 &  0.171 & 0.148 & T    \\
h300 & 43.171 & 0.149 & 53309.29 & 1.16   &   -7.334  &   19.862   &  -0.289 & 0.125 &  0.085 & 0.067 & T    \\
h311 & 43.498 & 0.141 & 53312.45 & 1.47   &   -7.628  &    7.158   &  -0.261 & 0.142 &  0.049 & 0.043 & F   \\
h319 & 42.609 & 0.165 & 53336.17 & 0.72   &   -8.755  &   31.473   &  -0.294 & 0.111 &  0.126 & 0.121 & T    \\
h323 & 43.092 & 0.181 & 53329.20 & 0.98   &   -8.792  &   13.120   &  -0.337 & 0.121 &  0.170 & 0.125 & T    \\
h359 & 41.980 & 0.270 & 53341.80 & 0.51   &   -9.439  &   29.126   &  -0.152 & 0.099 &  0.305 & 0.236 & T    \\
h363 & 40.212 & 0.309 & 53338.54 & 0.29   &  -12.724  &   38.444   &   0.149 & 0.117 &  0.923 & 0.315 & T    \\
h364 & 41.471 & 0.134 & 53333.58 & 0.48   &  -13.706  &   38.341   &  -0.053 & 0.102 &  0.083 & 0.085 & T    \\
k396 & 41.200 & 0.304 & 53358.22 & 0.92   &  -11.153  &    1.439   &  -0.032 & 0.398 &  0.157 & 0.152 & F   \\
k411 & 42.724 & 0.150 & 53340.64 & 0.82   &   -9.976  &   12.398   &  -0.257 & 0.133 &  0.099 & 0.092 & T    \\
k425 & 41.207 & 0.254 & 53335.19 & 0.43   &   -9.535  &   19.618   &  -0.087 & 0.177 &  0.310 & 0.236 & T    \\
k429 & 40.038 & 0.145 & 53350.08 & 0.45   &   -6.765  &   31.570   &  -0.135 & 0.090 &  0.153 & 0.140 & T    \\
k430 & 43.223 & 0.258 & 53348.34 & 2.37   &   -2.699  &    6.166   &  -0.061 & 0.269 &  0.170 & 0.127 & F   \\
k432 & 43.682 & 0.161 & 53335.68 & 1.74   &   -6.246  &    9.587   &  -0.237 & 0.163 &  0.065 & 0.055 & F   \\
k441 & 43.347 & 0.145 & 53354.55 & 1.63   &   -6.204  &   15.876   &  -0.273 & 0.137 &  0.089 & 0.066 & T    \\
k448 & 42.492 & 0.426 & 53355.36 & 1.84   &   -6.583  &    3.364   &   0.144 & 0.410 &  0.291 & 0.274 & F   \\
k467 & 43.201 & 0.154 & 53338.63 & 0.93   &   -8.394  &   12.142   &  -0.224 & 0.143 &  0.085 & 0.075 & T    \\
k485 & 42.292 & 0.398 & 53350.14 & 1.48   &   -4.219  &   20.355   &  -0.145 & 0.318 &  0.778 & 0.295 & T    \\
k490 & 43.675 & 0.148 & 53345.15 & 3.02   &   -0.569  &    7.570   &  -0.286 & 0.149 &  0.072 & 0.055 & F   \\
m001 & 41.058 & 0.180 & 53633.42 & 1.74   &    4.395  &   48.690   &   0.220 & 0.154 &  0.121 & 0.098 & F   \\
m022 & 41.474 & 0.358 & 53639.73 & 2.20   &   -0.586  &   55.088   &  -0.729 & 0.063 &  0.967 & 0.378 & F   \\
m026 & 43.240 & 0.216 & 53634.40 & 3.41   &    2.809  &    4.012   &  -0.150 & 0.209 &  0.098 & 0.074 & F   \\
m027 & 41.625 & 0.288 & 53639.87 & 1.52   &   -0.601  &   43.614   &  -0.078 & 0.187 &  0.363 & 0.276 & T    \\
m032 & 40.121 & 0.153 & 53632.12 & 2.05   &    5.953  &   89.121   &  -0.197 & 0.080 &  0.101 & 0.109 & F   \\
m034 & 42.670 & 0.268 & 53627.22 & 3.01   &    7.664  &   17.313   &  -0.116 & 0.213 &  0.140 & 0.148 & F   \\
m039 & 40.728 & 0.382 & 53626.03 & 2.29   &   10.521  &   64.211   &   0.163 & 0.256 &  0.262 & 0.282 & F   \\
m040 & 43.023 & 0.412 & 53642.75 & 3.16   &   -2.431  &   -2.404   &   0.074 & 0.343 &  0.232 & 0.203 & F   \\
m043 & 41.203 & 0.292 & 53640.46 & 1.11   &   -1.147  &   51.835   &  -0.604 & 0.058 &  1.206 & 0.294 & F   \\
m057 & 41.316 & 0.255 & 53631.49 & 2.35   &    8.158  &   90.255   &  -0.574 & 0.073 &  0.252 & 0.256 & F   \\
m062 & 41.489 & 0.265 & 53644.74 & 1.63   &   -2.786  &   45.173   &   0.021 & 0.269 &  0.191 & 0.171 & T    \\
m070 & 41.084 & 0.088 & 53641.82 & 1.06   &   -0.551  &   51.440   &  -0.246 & 0.087 &  0.046 & 0.041 & F   \\
m075 & 39.472 & 0.448 & 53640.71 & 1.15   &   -1.513  &   83.949   &  -0.663 & 0.048 &  1.516 & 0.497 & F   \\
m087 & 41.178 & 0.285 & 53636.35 & 2.23   &    3.734  &   52.696   &  -0.126 & 0.144 &  0.327 & 0.261 & T    \\
m138 & 42.932 & 0.228 & 53656.48 & 2.70   &   -4.663  &   -1.521   &  -0.043 & 0.229 &  0.084 & 0.084 & F   \\
m158 & 42.735 & 0.244 & 53656.72 & 1.77   &   -5.265  &   26.919   &  -0.243 & 0.167 &  0.159 & 0.151 & T    \\
m193 & 41.289 & 0.224 & 53663.09 & 0.58   &  -10.477  &   56.394   &  -0.075 & 0.143 &  0.132 & 0.104 & T    \\
m226 & 43.238 & 0.193 & 53651.66 & 2.18   &   -7.478  &    1.475   &  -0.213 & 0.205 &  0.099 & 0.080 & F   \\
n246 & 43.136 & 0.160 & 53708.26 & 1.79   &   -7.139  &   -0.091   &  -0.201 & 0.175 &  0.074 & 0.056 & F   \\
n256 & 43.154 & 0.140 & 53696.67 & 1.37   &   -8.911  &   10.678   &  -0.209 & 0.153 &  0.076 & 0.069 & T    \\
n258 & 42.847 & 0.226 & 53698.79 & 1.74   &   -1.761  &   19.279   &   0.018 & 0.241 &  0.098 & 0.103 & T    \\
n263 & 41.497 & 0.176 & 53703.71 & 0.71   &   -5.540  &   25.130   &   0.156 & 0.146 &  0.121 & 0.123 & T    \\
n278 & 41.165 & 0.207 & 53700.58 & 1.01   &   -1.955  &   26.436   &   0.087 & 0.201 &  0.190 & 0.155 & T    \\
n285 & 42.736 & 0.267 & 53688.64 & 1.80   &   -4.309  &   12.685   &  -0.118 & 0.226 &  0.149 & 0.157 & T    \\
n322 & 44.018 & 0.144 & 53709.35 & 2.49   &   -7.445  &   -0.669   &  -0.282 & 0.139 &  0.047 & 0.042 & F   \\
n326 & 40.624 & 0.279 & 53709.77 & 0.59   &   -9.296  &   16.839   &   0.899 & 0.236 &  0.203 & 0.187 & T    \\
n346 & 41.647 & 0.384 & 53683.16 & 1.74   &   -0.890  &   19.671   &   0.368 & 0.339 &  0.378 & 0.307 & T    \\
n400 & 43.221 & 0.407 & 53707.40 & 1.95   &   -5.082  &    3.304   &   0.109 & 0.373 &  0.257 & 0.254 & F   \\
n404 & 41.138 & 0.262 & 53713.62 & 0.42   &  -13.584  &   19.047   &  -0.124 & 0.154 &  0.405 & 0.258 & T    \\
p425 & 42.752 & 0.352 & 53696.76 & 2.76   &    0.874  &    7.754   &   0.027 & 0.337 &  0.263 & 0.232 & F   \\
p429 & 43.369 & 0.171 & 53710.18 & 2.10   &   -7.850  &   18.004   &  -0.478 & 0.098 &  0.114 & 0.110 & F   \\
p434 & 41.687 & 0.420 & 53704.07 & 1.43   &   -4.482  &    6.002   &   0.406 & 0.482 &  1.088 & 0.414 & F   \\
p444 & 43.613 & 0.200 & 53697.91 & 3.05   &    0.117  &    8.713   &  -0.162 & 0.211 &  0.115 & 0.089 & F   \\
p445 & 43.886 & 0.127 & 53702.17 & 3.30   &   -2.278  &    5.489   &  -0.318 & 0.120 &  0.043 & 0.031 & F   \\
p454 & 43.539 & 0.156 & 53703.60 & 2.41   &   -3.251  &    6.183   &  -0.211 & 0.169 &  0.078 & 0.059 & F   \\
p455 & 41.302 & 0.224 & 53721.63 & 0.44   &  -13.496  &   12.685   &  -0.193 & 0.197 &  0.208 & 0.175 & T    \\
p459 & 43.593 & 0.204 & 53692.29 & 3.40   &    3.415  &   12.787   &  -0.245 & 0.163 &  0.082 & 0.059 & T    \\
p524 & 42.642 & 0.165 & 53719.41 & 0.65   &  -11.397  &   12.370   &  -0.265 & 0.135 &  0.104 & 0.101 & T    \\
p528 & 43.661 & 0.117 & 53722.87 & 1.48   &  -10.514  &    8.529   &  -0.328 & 0.118 &  0.052 & 0.036 & F   \\
p534 & 42.926 & 0.211 & 53742.71 & 1.90   &   -9.012  &   -2.859   &  -0.105 & 0.227 &  0.104 & 0.085 & F   \\
q002 & 41.212 & 0.359 & 54002.83 & 0.75   &   -6.340  &   15.192   &   0.594 & 0.279 &  0.549 & 0.369 & T    \\
q006 & 41.846 & 0.358 & 53995.49 & 1.45   &   -0.944  &   21.547   &   0.376 & 0.384 &  0.198 & 0.205 & F   \\
q007 & 39.254 & 0.259 & 54000.19 & 0.77   &   -4.873  &   75.741   &  -0.133 & 0.082 &  1.990 & 0.266 & T    \\
q008 & 40.877 & 0.277 & 54005.99 & 0.38   &   -9.044  &   65.389   &  -0.046 & 0.083 &  0.446 & 0.265 & T    \\
q014 & 41.074 & 0.287 & 54006.35 & 0.49   &   -9.440  &   64.470   &  -0.318 & 0.064 &  0.581 & 0.290 & T    \\
q022 & 40.645 & 0.333 & 53991.76 & 2.01   &    0.429  &   55.001   &  -0.098 & 0.107 &  0.646 & 0.347 & T    \\
q048 & 42.017 & 0.338 & 54022.19 & 1.88   &   -0.669  &   20.049   &   0.325 & 0.327 &  0.270 & 0.242 & T    \\
q049 & 42.170 & 0.267 & 54015.38 & 0.77   &   -8.466  &   25.204   &  -0.188 & 0.145 &  0.256 & 0.220 & T    \\
q054 & 41.428 & 0.201 & 54024.27 & 1.18   &   -2.231  &   43.631   &  -0.165 & 0.098 &  0.225 & 0.171 & T    \\
q061 & 41.232 & 0.321 & 54026.58 & 1.19   &   -2.574  &   29.716   &  -0.129 & 0.168 &  1.249 & 0.283 & T    \\
q067 & 39.987 & 0.204 & 54033.25 & 0.33   &  -10.045  &   67.535   &  -0.256 & 0.060 &  0.221 & 0.205 & T    \\
q069 & 40.077 & 0.353 & 54005.53 & 1.74   &   14.027  &   63.815   &   0.610 & 0.250 &  0.174 & 0.199 & F   \\
q075 & 42.031 & 0.169 & 54017.44 & 0.63   &   -9.869  &   25.019   &  -0.175 & 0.119 &  0.112 & 0.116 & T    \\
q102 & 42.167 & 0.225 & 54030.72 & 0.92   &   -5.219  &   41.356   &  -0.192 & 0.121 &  0.209 & 0.182 & T    \\
q106 & 42.325 & 0.204 & 54036.39 & 0.72   &   -8.860  &   18.250   &  -0.067 & 0.168 &  0.131 & 0.130 & T    \\
q107 & 43.184 & 0.198 & 54034.39 & 1.46   &   -6.733  &   11.326   &  -0.116 & 0.198 &  0.102 & 0.075 & T    \\
q108 & 43.396 & 0.216 & 54016.42 & 1.38   &   -6.262  &    9.187   &  -0.188 & 0.208 &  0.113 & 0.107 & T    \\
q112 & 43.167 & 0.132 & 54032.05 & 1.65   &   -6.602  &   14.140   &  -0.324 & 0.122 &  0.093 & 0.075 & T    \\
q114 & 43.245 & 0.163 & 54037.82 & 1.86   &   -5.093  &   10.293   &  -0.209 & 0.172 &  0.080 & 0.061 & T    \\
q125 & 41.575 & 0.322 & 54000.53 & 2.55   &    1.992  &   28.698   &   0.014 & 0.173 &  0.384 & 0.262 & T    \\
r185 & 40.022 & 0.209 & 54052.35 & 0.51   &  -11.145  &   35.392   &   0.621 & 0.130 &  0.243 & 0.190 & F   \\
r186 & 40.906 & 0.194 & 54044.24 & 0.37   &  -11.389  &   51.696   &  -0.098 & 0.083 &  0.154 & 0.156 & T    \\
r190 & 41.790 & 0.209 & 54062.16 & 0.57   &   -8.168  &   25.068   &  -0.226 & 0.088 &  0.251 & 0.182 & T    \\
r193 & 43.137 & 0.116 & 54051.77 & 1.13   &   -8.946  &   23.787   &  -0.344 & 0.094 &  0.068 & 0.067 & T    \\
r195 & 42.836 & 0.244 & 54051.08 & 1.46   &   -8.942  &   10.472   &  -0.207 & 0.194 &  0.204 & 0.167 & T    \\
r196 & 41.755 & 0.416 & 54046.31 & 1.30   &   -7.167  &   36.366   &  -0.401 & 0.100 &  1.406 & 0.423 & F   \\
r199 & 42.165 & 0.348 & 54041.45 & 0.78   &  -10.005  &   35.984   &  -0.132 & 0.151 &  0.335 & 0.284 & T    \\
r200 & 40.678 & 0.313 & 54064.06 & 0.60   &   -8.613  &   14.070   &  -0.239 & 0.178 &  1.174 & 0.309 & T    \\
r206 & 43.132 & 0.178 & 54055.41 & 2.20   &   -1.471  &   21.524   &  -0.166 & 0.182 &  0.110 & 0.091 & T    \\
r207 & 42.759 & 0.216 & 54044.16 & 0.98   &   -8.239  &   14.801   &  -0.184 & 0.168 &  0.172 & 0.133 & T    \\
r209 & 42.142 & 0.200 & 54051.26 & 1.10   &   -8.290  &   29.672   &  -0.063 & 0.120 &  0.191 & 0.158 & T    \\
r212 & 43.298 & 0.209 & 54054.71 & 2.48   &   -0.980  &    7.573   &  -0.124 & 0.220 &  0.103 & 0.076 & F   \\
r213 & 41.460 & 0.277 & 54062.91 & 0.45   &   -7.394  &   37.834   &  -0.086 & 0.094 &  0.354 & 0.244 & T    \\
r225 & 41.862 & 0.413 & 54054.51 & 1.45   &   -2.405  &    7.592   &   0.579 & 0.438 &  0.583 & 0.351 & F   \\
r230 & 40.960 & 0.200 & 54070.37 & 0.31   &  -13.670  &   34.747   &  -0.176 & 0.079 &  0.288 & 0.194 & T    \\
r311 & 43.693 & 0.167 & 54057.31 & 3.66   &    3.270  &    4.391   &  -0.306 & 0.133 &  0.048 & 0.034 & F   \\
r317 & 43.619 & 0.153 & 54064.67 & 2.14   &   -6.703  &    1.469   &  -0.256 & 0.158 &  0.065 & 0.049 & F   \\
r318 & 40.117 & 0.178 & 54078.63 & 0.25   &  -15.872  &   28.222   &  -0.455 & 0.053 &  0.239 & 0.174 & F   \\
r322 & 42.621 & 0.178 & 54077.17 & 0.68   &   -9.209  &   24.376   &  -0.141 & 0.146 &  0.111 & 0.108 & T    \\
s340 & 42.706 & 0.224 & 54069.31 & 0.79   &  -10.629  &   16.825   &  -0.259 & 0.144 &  0.176 & 0.145 & T    \\
s346 & 41.455 & 0.237 & 54076.32 & 1.25   &   -5.599  &   28.924   &  -0.009 & 0.157 &  0.199 & 0.185 & T    \\
s347 & 41.502 & 0.228 & 54098.22 & 0.59   &  -10.772  &   12.067   &  -0.471 & 0.083 &  0.272 & 0.210 & F   \\
s349 & 40.801 & 0.278 & 54082.46 & 1.66   &    1.314  &   26.006   &   0.125 & 0.175 &  0.422 & 0.289 & T    \\
s350 & 43.500 & 0.148 & 54091.06 & 2.28   &   -5.303  &   11.914   &  -0.252 & 0.150 &  0.087 & 0.064 & T    \\
s351 & 43.860 & 0.170 & 54080.11 & 3.32   &    1.163  &    8.106   &  -0.275 & 0.152 &  0.068 & 0.052 & F   \\
s353 & 42.760 & 0.285 & 54068.94 & 2.98   &    8.359  &   15.976   &  -0.131 & 0.219 &  0.144 & 0.144 & F   \\
s354 & 43.298 & 0.136 & 54081.85 & 1.40   &  -10.649  &   20.672   &  -0.415 & 0.081 &  0.103 & 0.097 & F   \\
s355 & 43.588 & 0.145 & 54090.11 & 2.05   &   -4.785  &   12.577   &  -0.254 & 0.147 &  0.080 & 0.062 & T    \\
s370 & 42.380 & 0.176 & 54095.61 & 1.03   &   -7.957  &   12.175   &  -0.221 & 0.162 &  0.115 & 0.115 & T    \\
s372 & 43.689 & 0.153 & 54088.34 & 2.83   &   -3.646  &    3.395   &  -0.214 & 0.167 &  0.066 & 0.054 & F   \\
s373 & 43.589 & 0.165 & 54090.14 & 2.42   &   -4.862  &   13.914   &  -0.168 & 0.174 &  0.071 & 0.062 & T    \\
s374 & 43.910 & 0.134 & 54090.61 & 3.39   &   -1.398  &    2.037   &  -0.265 & 0.149 &  0.054 & 0.045 & F   \\
s375 & 42.609 & 0.208 & 54101.27 & 0.73   &   -8.442  &    8.232   &  -0.264 & 0.170 &  0.138 & 0.137 & F   \\
s377 & 41.434 & 0.330 & 54082.37 & 1.22   &   -9.418  &   22.653   &  -0.189 & 0.139 &  0.504 & 0.308 & T    \\
s379 & 40.394 & 0.194 & 54102.08 & 0.36   &  -13.444  &   10.044   &  -0.435 & 0.090 &  0.265 & 0.201 & F   \\
s380 & 43.411 & 0.240 & 54099.42 & 1.29   &   -8.141  &    8.376   &  -0.144 & 0.241 &  0.148 & 0.107 & F   \\
x016 & 42.189 & 0.399 & 54370.25 & 0.88   &   -7.399  &   12.649   &   0.296 & 0.365 &  0.332 & 0.336 & T    \\
x017 & 41.829 & 0.311 & 54374.82 & 2.54   &    1.682  &   52.180   &  -0.279 & 0.116 &  0.426 & 0.288 & T    \\
x020 & 43.578 & 0.207 & 54370.41 & 2.25   &   -4.272  &    7.824   &  -0.145 & 0.208 &  0.096 & 0.075 & F   \\
x025 & 41.588 & 0.284 & 54357.28 & 1.51   &   -4.435  &   61.817   &   0.031 & 0.201 &  0.256 & 0.245 & T    \\
x028 & 43.033 & 0.194 & 54369.71 & 1.05   &   -9.637  &    8.456   &  -0.187 & 0.192 &  0.112 & 0.096 & F   \\
x033 & 41.925 & 0.230 & 54388.66 & 0.99   &   -6.714  &   35.866   &  -0.077 & 0.160 &  0.125 & 0.127 & T    \\
x034 & 42.507 & 0.302 & 54372.23 & 1.13   &   -5.814  &   13.751   &   0.193 & 0.259 &  0.204 & 0.177 & T    \\
x038 & 42.607 & 0.289 & 54383.77 & 2.17   &   -5.579  &   36.515   &  -0.455 & 0.085 &  0.336 & 0.234 & F   \\
x039 & 42.656 & 0.117 & 54376.29 & 1.37   &   -9.007  &   21.942   &  -0.284 & 0.105 &  0.046 & 0.042 & T    \\
x055 & 40.887 & 0.188 & 54371.71 & 0.37   &  -12.846  &   54.432   &   0.105 & 0.112 &  0.163 & 0.134 & T    \\
x066 & 41.329 & 0.184 & 54354.28 & 1.26   &   -2.225  &   51.916   &  -0.090 & 0.101 &  0.157 & 0.136 & T    \\
x071 & 42.636 & 0.169 & 54393.83 & 0.67   &   -9.796  &   19.802   &  -0.196 & 0.132 &  0.107 & 0.104 & T    \\
x077 & 42.659 & 0.180 & 54388.69 & 1.14   &   -4.845  &   22.788   &  -0.261 & 0.102 &  0.160 & 0.132 & T    \\
x080 & 42.006 & 0.440 & 54384.94 & 1.54   &   -4.178  &   17.699   &   0.132 & 0.343 &  0.315 & 0.276 & T    \\
x085 & 43.257 & 0.186 & 54392.38 & 1.50   &   -6.756  &    0.600   &  -0.133 & 0.207 &  0.091 & 0.075 & F   \\
x089 & 42.998 & 0.411 & 54387.22 & 1.89   &   -6.629  &    4.026   &  -0.117 & 0.308 &  0.352 & 0.269 & F   \\
x093 & 43.161 & 0.425 & 54385.69 & 2.25   &   -2.905  &    5.111   &  -0.006 & 0.353 &  0.306 & 0.248 & F   \\
x107 & 39.579 & 0.148 & 54404.07 & 0.30   &  -14.616  &   56.773   &  -0.232 & 0.061 &  0.155 & 0.142 & T    \\
y125 & 41.318 & 0.175 & 54412.02 & 0.62   &  -14.306  &   29.819   &  -0.124 & 0.103 &  0.175 & 0.150 & T    \\
y127 & 42.765 & 0.137 & 54405.28 & 0.88   &   -8.964  &   23.123   &  -0.304 & 0.091 &  0.090 & 0.089 & T    \\
y134 & 41.649 & 0.141 & 54412.48 & 1.28   &   -2.480  &   20.175   &  -0.296 & 0.116 &  0.119 & 0.115 & T    \\
y136 & 42.422 & 0.288 & 54411.89 & 1.72   &   -1.695  &   21.866   &  -0.425 & 0.096 &  0.719 & 0.241 & F   \\
y137 & 41.804 & 0.181 & 54418.70 & 0.64   &   -8.343  &   36.654   &  -0.188 & 0.097 &  0.153 & 0.139 & T    \\
y142 & 42.728 & 0.185 & 54421.15 & 0.90   &   -7.482  &   17.714   &  -0.173 & 0.133 &  0.134 & 0.123 & T    \\
y143 & 42.544 & 0.164 & 54404.78 & 1.05   &   -7.873  &   30.295   &  -0.296 & 0.080 &  0.143 & 0.130 & T    \\
y145 & 42.754 & 0.137 & 54418.78 & 1.02   &   -7.460  &   14.363   &  -0.303 & 0.109 &  0.090 & 0.089 & T    \\
y151 & 42.992 & 0.184 & 54427.39 & 0.77   &  -11.427  &   13.735   &  -0.226 & 0.147 &  0.152 & 0.114 & T    \\
y154 & 43.202 & 0.154 & 54419.41 & 1.41   &   -6.141  &   11.909   &  -0.067 & 0.154 &  0.061 & 0.046 & T    \\
y155 & 41.642 & 0.087 & 54436.58 & 0.71   &  -11.832  &    7.948   &  -0.361 & 0.087 &  0.035 & 0.028 & F   \\
y158 & 42.588 & 0.191 & 54422.53 & 0.68   &   -8.936  &   17.897   &  -0.201 & 0.128 &  0.179 & 0.141 & T    \\
y163 & 43.662 & 0.196 & 54421.29 & 2.33   &   -6.154  &   12.159   &  -0.255 & 0.182 &  0.134 & 0.107 & T    \\
y175 & 41.655 & 0.268 & 54425.80 & 0.53   &  -11.680  &   16.528   &   0.548 & 0.197 &  0.221 & 0.226 & T    \\
y177 & 41.024 & 0.263 & 54436.17 & 0.29   &  -14.572  &   27.576   &  -0.311 & 0.074 &  0.383 & 0.245 & T    \\
z180 & 42.002 & 0.207 & 54441.79 & 1.04   &   -4.577  &   22.144   &  -0.138 & 0.131 &  0.211 & 0.174 & T    \\
z181 & 43.246 & 0.173 & 54438.53 & 2.30   &   -2.072  &   17.656   &  -0.206 & 0.184 &  0.117 & 0.092 & T    \\
z183 & 41.083 & 0.118 & 54436.07 & 0.46   &  -11.691  &   29.514   &  -0.210 & 0.072 &  0.105 & 0.098 & T    \\
z185 & 42.107 & 0.174 & 54430.83 & 0.79   &   -6.969  &   29.321   &   0.027 & 0.130 &  0.104 & 0.115 & T    \\
z187 & 41.138 & 0.203 & 54441.72 & 0.56   &  -14.291  &   24.965   &   0.035 & 0.105 &  0.218 & 0.188 & F   \\
z200 & 42.427 & 0.271 & 54452.44 & 0.66   &   -7.845  &   14.853   &  -0.033 & 0.225 &  0.217 & 0.187 & T    \\
z202 & 40.360 & 0.188 & 54448.76 & 0.38   &   -9.484  &   20.771   &  -0.130 & 0.120 &  0.219 & 0.187 & T    \\
z203 & 42.479 & 0.324 & 54451.19 & 0.64   &   -9.647  &   18.344   &  -0.214 & 0.176 &  0.426 & 0.337 & T    \\
z204 & 43.125 & 0.194 & 54452.72 & 0.86   &   -8.386  &   10.128   &  -0.132 & 0.191 &  0.103 & 0.085 & T    \\
z205 & 41.843 & 0.291 & 54452.83 & 0.55   &   -9.736  &   13.767   &  -0.229 & 0.164 &  0.299 & 0.249 & T    \\
z208 & 42.807 & 0.156 & 54454.79 & 0.68   &   -8.995  &   12.590   &  -0.264 & 0.132 &  0.109 & 0.102 & T    \\
\end{longtable}                                           

\tablenotetext{a}{MLCS2k2 reports distance moduli with H$_{0} = 65$~km s$^{-1}$ Mpc$^{-1}$.}
\tablenotetext{b}{$\Phi_{\text{First|Last}}$ is the rest-frame phase of the first and last observation (respectively) and is dependent on the $B$-band time of maximum brightness, $T^{B}_{max}$. }
\tablenotetext{c}{Mag units. We use the Galactic reddening law of \citet{odonnell94}, with $R_{V}$ fixed to 3.1, to model the extinction in the host galaxy of the SN.}
\tablenotetext{d}{Flag describing if the object passes (T) or fails (F) the light-curve quality cuts described by WV07.}

\end{center}
%\end{landscape}
\onehalfspacing


==> SALT2_fitp.tex <==
\begin{landscape}
\begin{center}
\singlespacing
\scriptsize
%\begin{longtable}{lccccccrcrcrc}
\begin{longtable}{ccccccccccccc}
\caption{SALT2 Light-Curve Fit Parameters for ESSENCE \snia\ and ``Ia?'' Objects\label{tab:SALT2fitp}}\\

\hline \hline
ID &
$m_{B}$\tablenotemark{a} &
$\sigma_{m_{B}}$ &
$m_{V}$ &
$\sigma_{m_{V}}$ &
$T^{B}_{\text{max}}$\tablenotemark{b}&
$\sigma_{T^{B}_{\text{max}}}$ &
$x_{1}$ &
$\sigma_{x_{1}}$ &
$c$\tablenotemark{c} &
$\sigma_{c}$ &
${\rm Cov}(c,x_{1})$\tablenotemark{d}&
Q\tablenotemark{e} \\
\hline
\endfirsthead

\multicolumn{13}{c}%
{{\bfseries \tablename\ \thetable{} (Continued)}} \\
%{{\bfseries \tablename\ \thetable{} --- continued from previous page}} \\

\hline
ID &
$m_{B}$\tablenotemark{a} &
$\sigma_{m_{B}}$ &
$m_{V}$ &
$\sigma_{m_{V}}$ &
$T^{B}_{\text{max}}$\tablenotemark{b}&
$\sigma_{T^{B}_{\text{max}}}$ &
$x_{1}$ &
$\sigma_{x_{1}}$ &
$c$\tablenotemark{c} &
$\sigma_{c}$ &
${\rm Cov}(c,x_{1})$\tablenotemark{d}&
Q\tablenotemark{e} \\
\hline
\endhead

\hline \multicolumn{13}{c}{{Continued on next page}} \\ \hline
\endfoot

\hline
\hline
\endlastfoot
b010 & 23.4583 & 0.0666 & 23.5138 & 0.0937 & 52593.2578 & 0.8841 &  0.9105 & 0.7618 & -0.0781 & 0.1012 &  0.0248 & T     \\
b013 & 22.6982 & 0.0441 & 22.6821 & 0.0343 & 52588.2349 & 0.6787 & -0.1382 & 0.4106 & -0.0069 & 0.0553 & -0.0015 & T     \\
b016 & 22.5752 & 0.1009 & 22.4429 & 0.0410 & 52584.7886 & 1.4696 &  0.4887 & 0.8185 &  0.1069 & 0.0889 &  0.0066 & T     \\
b017 & 21.4923 & 0.0797 & 21.4956 & 0.0352 & 52595.4475 & 0.2830 & -0.2884 & 0.3204 & -0.0260 & 0.0609 &  0.0035 & T     \\
b020 & 22.7302 & 0.0822 & 22.6162 & 0.0900 & 52601.8351 & 0.9118 &  0.8373 & 0.9984 &  0.0886 & 0.0887 & -0.0035 & F    \\
b022 & 23.1333 & 0.0626 & 23.4180 & 0.0843 & 52596.2911 & 0.6042 & -1.1228 & 0.5926 & -0.3011 & 0.0913 &  0.0060 & F    \\
c015 & 23.2594 & 0.0872 & 23.1716 & 0.0469 & 52619.0456 & 0.5744 &  0.4944 & 0.5771 &  0.0630 & 0.0865 &  0.0125 & T     \\
d033 & 23.4614 & 0.0637 & 23.3019 & 0.0826 & 52936.7009 & 1.9256 &  3.3665 & 0.9741 &  0.1311 & 0.0958 & -0.0139 & F    \\
d058 & 23.6319 & 0.0678 & 23.2789 & 0.1034 & 52941.9994 & 1.0806 &  1.2436 & 0.7267 &  0.3238 & 0.1057 & -0.0035 & F    \\
d083 & 21.0610 & 0.0479 & 21.1507 & 0.0225 & 52938.2117 & 0.4522 &  1.2102 & 0.1921 & -0.1119 & 0.0449 & -0.0009 & F    \\
d084 & 23.6840 & 0.0580 & 23.5824 & 0.0863 & 52936.2854 & 1.1608 & -0.8144 & 0.8059 &  0.0777 & 0.0989 & -0.0119 & T     \\
d085 & 22.4700 & 0.0528 & 22.4655 & 0.0452 & 52942.7811 & 0.3767 &  0.8873 & 0.3907 & -0.0192 & 0.0619 & -0.0038 & T     \\
d086 & 20.9939 & 0.0743 & 20.9406 & 0.0257 & 52947.0097 & 0.1326 &  0.0660 & 0.1678 &  0.0294 & 0.0575 &  0.0003 & T     \\
d089 & 22.4754 & 0.0474 & 22.5214 & 0.0372 & 52929.4122 & 0.6286 &  0.4573 & 0.3600 & -0.0684 & 0.0574 & -0.0027 & T     \\
d093 & 21.9899 & 0.0540 & 22.0881 & 0.0307 & 52949.4497 & 0.2449 &  1.1777 & 0.2756 & -0.1201 & 0.0506 &  0.0017 & T     \\
d097 & 22.5686 & 0.0449 & 22.6021 & 0.0363 & 52939.6901 & 0.4616 &  1.1890 & 0.3218 & -0.0567 & 0.0546 & -0.0025 & T     \\
d099 & 20.9724 & 0.0986 & 21.0124 & 0.0606 & 52918.3226 & 0.6958 &  2.0693 & 0.5334 & -0.0639 & 0.0817 & -0.0178 & F    \\
d100 & 20.0110 & 0.1119 & 19.8475 & 0.0424 & 52929.2329 & 0.9004 &  2.1698 & 0.3017 &  0.1361 & 0.0869 & -0.0066 & F    \\
d117 & 22.3145 & 0.0862 & 22.3156 & 0.0388 & 52949.1832 & 0.2747 & -1.7648 & 0.3176 & -0.0225 & 0.0711 &  0.0049 & T     \\
d149 & 22.1197 & 0.0523 & 22.0998 & 0.0307 & 52955.8454 & 0.2586 &  0.0015 & 0.2362 & -0.0033 & 0.0478 & -0.0007 & T     \\
e020 & 21.7497 & 0.2797 & 21.0455 & 0.0744 & 52974.3431 & 0.8528 &  3.8656 & 1.0929 &  0.6702 & 0.2220 &  0.0927 & F    \\
e108 & 22.7046 & 0.0571 & 22.7138 & 0.0504 & 52982.0137 & 0.7895 &  2.8731 & 0.9164 & -0.0343 & 0.0672 &  0.0176 & F    \\
e132 & 21.6510 & 0.0584 & 21.5453 & 0.0201 & 52973.6715 & 0.1880 &  0.0844 & 0.1908 &  0.0810 & 0.0482 &  0.0017 & T     \\
e136 & 22.7645 & 0.0494 & 22.6838 & 0.0261 & 52967.9480 & 0.5024 & -0.7407 & 0.3937 &  0.0571 & 0.0514 & -0.0007 & T     \\
e138 & 24.0052 & 0.0848 & 23.5880 & 0.1539 & 52958.8777 & 0.9445 &  3.7621 & 1.0456 &  0.3851 & 0.1367 & -0.0316 & F    \\
e140 & 23.3562 & 0.0371 & 23.3736 & 0.0748 & 52972.6678 & 0.6435 & -0.5625 & 0.4455 & -0.0395 & 0.0767 &  0.0014 & T     \\
e147 & 23.4887 & 0.0432 & 23.5845 & 0.0835 & 52964.0667 & 0.6514 &  0.8702 & 0.4969 & -0.1176 & 0.0790 &  0.0038 & T     \\
e148 & 22.7213 & 0.0417 & 22.7610 & 0.0327 & 52977.7135 & 0.2648 &  0.2216 & 0.2999 & -0.0621 & 0.0490 & -0.0002 & F    \\
e149 & 22.9999 & 0.0611 & 23.1688 & 0.0562 & 52952.4141 & 0.3075 & -0.2293 & 0.3723 & -0.1884 & 0.0710 &  0.0072 & T     \\
f011 & 23.1913 & 0.0508 & 23.3118 & 0.0617 & 52985.3738 & 0.6284 & -0.7538 & 0.4554 & -0.1406 & 0.0737 &  0.0067 & T     \\
f041 & 23.2151 & 0.0547 & 23.3547 & 0.0733 & 52989.6182 & 1.1049 &  2.5583 & 0.9827 & -0.1617 & 0.0759 &  0.0120 & F    \\
f096 & 22.4723 & 0.7368 & 22.7005 & 0.0751 & 52993.6277 & 1.6711 & -0.1097 & 2.4140 & -0.2466 & 0.6468 &  0.2074 & F    \\
f123 & 23.6000 & 0.0677 & 23.5107 & 0.0941 & 52988.7551 & 0.8700 & -0.4000 & 0.7952 &  0.0652 & 0.1026 &  0.0085 & T     \\
f216 & 23.6903 & 0.1012 & 23.9354 & 0.1618 & 52984.1900 & 0.7385 & -3.2609 & 0.8793 & -0.2608 & 0.1657 &  0.0344 & F    \\
f231 & 23.5144 & 0.0789 & 23.4800 & 0.1066 & 52990.3566 & 1.6953 &  3.7531 & 1.8284 &  0.0078 & 0.1093 &  0.0752 & F    \\
f235 & 22.4115 & 0.0458 & 22.5296 & 0.0349 & 52989.9928 & 0.4777 & -0.3129 & 0.4195 & -0.1385 & 0.0549 &  0.0004 & F    \\
f244 & 23.3649 & 0.0592 & 23.3709 & 0.0783 & 52986.1800 & 0.9165 & -0.3328 & 0.7171 & -0.0285 & 0.0896 &  0.0081 & T     \\
f301 & 23.8662 & 0.0705 & 23.5720 & 0.1076 & 53003.2781 & 1.2802 &  5.0000 & 1.6537 &  0.2625 & 0.1239 &  0.0000 & F    \\
f308 & 22.9912 & 0.0604 & 23.0399 & 0.0445 & 52996.3113 & 2.1191 &  1.4827 & 1.8214 & -0.0719 & 0.0721 &  0.0117 & F    \\
g001 & 21.5380 & 0.0641 & 21.5587 & 0.0276 & 53286.0117 & 0.5405 & -0.7699 & 0.2664 & -0.0426 & 0.0523 &  0.0004 & F    \\
g005 & 21.2137 & 0.0719 & 21.0864 & 0.0244 & 53295.0501 & 0.3713 &  1.3354 & 0.2449 &  0.1011 & 0.0585 & -0.0009 & T     \\
g050 & 23.2239 & 0.0702 & 23.4278 & 0.1084 & 53302.2280 & 0.5811 & -0.2400 & 0.5682 & -0.2226 & 0.1069 &  0.0153 & T     \\
g052 & 22.4627 & 0.0631 & 22.4921 & 0.0403 & 53297.1287 & 0.4029 & -1.1883 & 0.3363 & -0.0507 & 0.0704 & -0.0003 & T     \\
g053 & 23.4662 & 0.0648 & 23.6604 & 0.1395 & 53287.0857 & 1.1470 & -0.0611 & 0.6761 & -0.2132 & 0.1209 &  0.0080 & T     \\
g055 & 23.2292 & 0.1051 & 22.7479 & 0.0403 & 53289.7042 & 0.9378 &  0.2126 & 0.5193 &  0.4517 & 0.0832 &  0.0030 & F    \\
g097 & 22.3097 & 0.0847 & 22.1334 & 0.0428 & 53300.8226 & 0.4055 &  1.6368 & 0.4938 &  0.1491 & 0.0700 &  0.0085 & T     \\
g120 & 22.8643 & 0.0446 & 22.8299 & 0.0533 & 53298.9711 & 0.6943 &  0.3097 & 0.4151 &  0.0106 & 0.0685 & -0.0004 & T     \\
g133 & 21.7833 & 0.2214 & 22.2327 & 0.0877 & 53272.8899 & 0.9993 & -0.4481 & 0.8376 & -0.4625 & 0.1532 &  0.0928 & F    \\
g142 & 23.2658 & 0.0817 & 23.1028 & 0.0492 & 53296.3777 & 0.7751 & -1.3548 & 0.6054 &  0.1387 & 0.0898 & -0.0040 & T     \\
g160 & 22.9379 & 0.0570 & 22.9323 & 0.0657 & 53285.1450 & 0.6304 &  1.6888 & 0.4974 & -0.0188 & 0.0767 &  0.0018 & T     \\
g225 & 23.8654 & 0.0637 & 23.8810 & 0.1301 & 53334.2791 & 2.2526 &  5.0000 & 1.1594 & -0.0422 & 0.1318 &  0.0000 & F    \\
g230 & 22.8274 & 0.1199 & 22.9291 & 0.0878 & 53310.6496 & 0.4415 & -0.2586 & 0.5898 & -0.1225 & 0.0990 &  0.0022 & F    \\
g240 & 23.3988 & 0.0952 & 23.5517 & 0.1200 & 53307.0413 & 0.6828 &  0.1855 & 0.8960 & -0.1731 & 0.1016 &  0.0341 & T     \\
h283 & 23.3473 & 0.0514 & 23.3307 & 0.0628 & 53321.2118 & 0.9090 & -0.5594 & 0.5436 & -0.0062 & 0.0795 & -0.0018 & T     \\
h300 & 23.5692 & 0.0792 & 23.6237 & 0.1248 & 53310.9055 & 0.7499 &  1.7150 & 0.8095 & -0.0777 & 0.0984 &  0.0069 & T     \\
h311 & 23.8232 & 0.0950 & 23.9011 & 0.1650 & 53315.3237 & 1.0857 &  2.6953 & 1.0677 & -0.1015 & 0.1243 &  0.0205 & F    \\
h319 & 22.9405 & 0.0503 & 23.0163 & 0.0509 & 53337.7782 & 0.4908 &  1.2528 & 0.5071 & -0.0983 & 0.0629 &  0.0038 & T     \\
h323 & 23.4921 & 0.0594 & 23.3174 & 0.0873 & 53329.8365 & 0.6337 &  0.6074 & 0.5493 &  0.1485 & 0.0930 &  0.0094 & F    \\
h359 & 22.6038 & 0.0520 & 22.5678 & 0.0275 & 53342.9415 & 0.3482 &  0.2210 & 0.2660 &  0.0123 & 0.0514 & -0.0009 & T     \\
h363 & 21.8893 & 0.0760 & 21.6406 & 0.0257 & 53339.2308 & 0.1866 & -0.7550 & 0.1842 &  0.2226 & 0.0613 & -0.0006 & T     \\
h364 & 21.7670 & 0.0491 & 21.8908 & 0.0259 & 53334.0477 & 0.1977 &  0.2617 & 0.2306 & -0.1446 & 0.0468 &  0.0010 & T     \\
k396 & 21.7503 & 0.0946 & 21.7029 & 0.0391 & 53361.2948 & 1.0275 &  1.9752 & 0.8884 &  0.0221 & 0.0834 &  0.0429 & F    \\
k411 & 23.0522 & 0.0511 & 23.1933 & 0.0760 & 53342.7973 & 0.7353 &  1.5361 & 0.7139 & -0.1625 & 0.0797 &  0.0045 & T     \\
k425 & 21.9104 & 0.0622 & 21.8304 & 0.0256 & 53336.3330 & 0.2477 & -0.2448 & 0.2967 &  0.0560 & 0.0514 &  0.0020 & T     \\
k429 & 20.4364 & 0.0839 & 20.4809 & 0.0269 & 53351.0711 & 0.1812 &  0.3730 & 0.1418 & -0.0669 & 0.0633 & -0.0004 & T     \\
k430 & 23.7691 & 0.0555 & 23.6982 & 0.0985 & 53347.5867 & 1.2664 & -0.6160 & 0.9686 &  0.0473 & 0.1047 &  0.0014 & T     \\
k432 & 23.8125 & 0.1445 & 24.0866 & 0.1583 & 53335.6225 & 0.9447 & -1.5615 & 1.3778 & -0.2905 & 0.1630 &  0.1419 & F    \\
k441 & 23.6810 & 0.0454 & 23.6852 & 0.1004 & 53355.8840 & 1.0612 &  1.0498 & 0.6641 & -0.0278 & 0.0849 &  0.0076 & T     \\
k448 & 23.4709 & 0.0879 & 23.2815 & 0.0589 & 53357.0838 & 1.5019 & -0.3872 & 1.1569 &  0.1639 & 0.1002 & -0.0058 & T     \\
k467 & 23.5194 & 0.0729 & 23.7493 & 0.1072 & 53340.9072 & 0.7840 &  0.6415 & 0.6746 & -0.2487 & 0.0934 &  0.0124 & T     \\
k485 & 23.7586 & 0.0685 & 23.3314 & 0.0490 & 53350.0235 & 0.8867 & -1.4635 & 0.9912 &  0.3995 & 0.0831 & -0.0091 & F    \\
k490 & 23.9589 & 0.0676 & 23.8262 & 0.1333 & 53349.2034 & 1.4763 &  0.0667 & 1.0362 &  0.1075 & 0.1082 &  0.0221 & T     \\
m001 & 21.7235 & 0.0953 & 21.7998 & 0.0438 & 53637.6811 & 0.9515 & -2.1337 & 0.4151 & -0.0961 & 0.0747 & -0.0031 & F    \\
m022 & 22.8951 & 0.1052 & 22.5488 & 0.0396 & 53641.3330 & 1.2189 &  0.9313 & 0.6791 &  0.3174 & 0.0827 &  0.0040 & F    \\
m026 & 22.3500 & 0.4535 & 23.1400 & 0.2375 & 53616.0645 & 3.2559 & -1.6072 & 1.4118 & -0.7934 & 0.3960 &  0.4653 & F    \\
m027 & 22.5307 & 0.1123 & 22.3609 & 0.0460 & 53641.3247 & 1.3194 &  0.2608 & 0.8020 &  0.1439 & 0.0829 & -0.0070 & F    \\
m032 & 20.5396 & 0.1368 & 20.5039 & 0.0754 & 53632.4770 & 2.4228 &  1.2530 & 0.9453 &  0.0111 & 0.1052 &  0.0243 & F    \\
m034 & 23.2896 & 0.1959 & 23.0804 & 0.1311 & 53627.4271 & 4.8914 &  1.5744 & 1.5743 &  0.1816 & 0.1644 &  0.0460 & F    \\
m039 & 21.9462 & 0.1211 & 21.7622 & 0.0889 & 53631.8543 & 2.1447 & -1.1710 & 0.8505 &  0.1592 & 0.0754 &  0.0171 & F    \\
m040 & 22.1793 & 0.7274 & 23.1579 & 0.2103 & 53621.6532 & 2.7408 & -3.5000 & 0.7281 & -0.9763 & 0.5939 &  0.3171 & F    \\
m043 & 23.1040 & 0.1207 & 22.5762 & 0.0455 & 53639.2515 & 1.4737 &  5.0000 & 0.7916 &  0.4937 & 0.1035 &  0.0000 & F    \\
m057 & 22.4255 & 0.1850 & 22.0259 & 0.0622 & 53639.6535 & 1.1983 &  1.8654 & 1.0813 &  0.3693 & 0.1470 &  0.0519 & F    \\
m062 & 22.0414 & 0.0928 & 22.0845 & 0.0449 & 53644.8605 & 1.0827 & -1.3465 & 1.0464 & -0.0641 & 0.0769 &  0.0150 & T     \\
m070 & 19.5829 & 0.1687 & 20.4357 & 0.0811 & 53622.0860 & 1.7494 &  0.8312 & 0.4625 & -0.8547 & 0.1009 &  0.0053 & F    \\
m075 & 26.2051 & 0.0505 & 22.3018 & 0.0502 & 53640.3370 & 1.0284 &  1.8606 & 0.5860 &  4.0000 & 1.6263 &  0.0000 & F    \\
m087 & 21.9348 & 0.0714 & 21.8453 & 0.0368 & 53639.1987 & 1.4325 & -0.3253 & 0.8816 &  0.0654 & 0.0591 &  0.0050 & F    \\
m138 & 23.3608 & 0.1017 & 23.6810 & 0.1609 & 53658.3095 & 1.5835 &  1.5827 & 1.1046 & -0.3375 & 0.1286 &  0.0054 & F    \\
m158 & 23.0549 & 0.0782 & 23.1014 & 0.0795 & 53659.6888 & 0.6083 &  0.9868 & 0.6352 & -0.0693 & 0.0905 &  0.0008 & T     \\
m193 & 21.5612 & 0.0833 & 21.6825 & 0.0549 & 53664.1930 & 0.1994 & -0.3418 & 0.2990 & -0.1417 & 0.0570 &  0.0024 & T     \\
m226 & 23.6021 & 0.0708 & 23.2621 & 0.1581 & 53651.3938 & 2.0210 &  0.6357 & 1.0882 &  0.3115 & 0.1544 &  0.0377 & F    \\
n246 & 23.3812 & 0.0748 & 23.3462 & 0.1746 & 53709.8276 & 0.9684 &  0.4924 & 0.6411 &  0.0110 & 0.1179 &  0.0113 & T     \\
n256 & 23.4379 & 0.0438 & 23.5728 & 0.0813 & 53697.9705 & 0.9806 &  0.8878 & 0.6175 & -0.1558 & 0.0789 &  0.0092 & T     \\
n258 & 23.2428 & 0.0393 & 23.4242 & 0.0639 & 53699.3885 & 0.6790 & -0.9953 & 0.5138 & -0.2000 & 0.0719 & -0.0018 & F    \\
n263 & 22.0192 & 0.0425 & 22.1161 & 0.0238 & 53703.6252 & 0.2486 & -0.6489 & 0.2685 & -0.1174 & 0.0452 & -0.0005 & T     \\
n278 & 21.7854 & 0.0506 & 21.8036 & 0.0220 & 53701.5420 & 0.5195 & -1.0085 & 0.5638 & -0.0399 & 0.0475 &  0.0034 & T     \\
n285 & 23.2297 & 0.0972 & 23.1655 & 0.0961 & 53689.6364 & 1.2069 &  0.2228 & 1.1534 &  0.0400 & 0.1161 &  0.0674 & T     \\
n322 & 24.3561 & 0.0919 & 24.4587 & 0.2019 & 53707.8798 & 1.4726 &  0.1779 & 1.0967 & -0.1237 & 0.1342 &  0.0518 & T     \\
n326 & 22.0658 & 0.1151 & 22.0876 & 0.0435 & 53709.2121 & 0.4490 & -3.7617 & 0.5910 & -0.0413 & 0.0948 &  0.0161 & F    \\
n400 & 24.0897 & 0.1003 & 23.9321 & 0.0920 & 53707.0709 & 1.7317 & -4.1715 & 5.1853 &  0.1357 & 0.1393 &  0.0160 & F    \\
n404 & 21.8702 & 0.0802 & 21.7000 & 0.0258 & 53714.0553 & 0.2202 & -0.1815 & 0.2845 &  0.1448 & 0.0627 &  0.0067 & T     \\
n406 & 23.8601 & 0.0705 & 24.0906 & 0.1329 & 53715.0012 & 0.7150 &  0.1731 & 0.5746 & -0.2489 & 0.0859 &  0.0103 & T     \\
p425 & 23.6726 & 0.0776 & 23.5157 & 0.0756 & 53700.3857 & 1.5386 &  1.4599 & 1.4828 &  0.1302 & 0.0998 &  0.0239 & T     \\
p429 & 23.9145 & 0.0604 & 23.7990 & 0.1366 & 53713.6481 & 1.7484 &  5.0000 & 0.9107 &  0.0863 & 0.1382 &  0.0000 & F    \\
p434 & 24.3087 & 0.2358 & 23.5397 & 0.0892 & 53710.4678 & 4.3975 &  4.9364 & 9.3685 &  0.7339 & 0.2248 &  0.4241 & F    \\
p444 & 24.0781 & 0.0784 & 23.9370 & 0.1270 & 53699.1613 & 2.1878 &  0.9862 & 1.0074 &  0.1151 & 0.1204 &  0.0204 & T     \\
p445 & 24.2080 & 0.0729 & 24.3789 & 0.1568 & 53705.4561 & 2.2305 &  0.5518 & 1.6851 & -0.1909 & 0.1060 &  0.0777 & T     \\
p454 & 23.8985 & 0.0487 & 23.8752 & 0.1094 & 53706.3840 & 1.5493 &  0.5749 & 0.8033 & -0.0005 & 0.0923 &  0.0092 & T     \\
p455 & 21.6367 & 0.0534 & 21.7212 & 0.0252 & 53721.6950 & 0.1964 & -0.7354 & 0.2612 & -0.1052 & 0.0454 &  0.0018 & T     \\
p459 & 23.9485 & 0.1308 & 23.7126 & 0.1643 & 53696.8230 & 3.2608 & -0.8275 & 1.0894 &  0.2101 & 0.1439 &  0.0307 & T     \\
p524 & 23.0226 & 0.0783 & 23.0937 & 0.0757 & 53721.0248 & 0.4854 &  1.8509 & 0.7723 & -0.0942 & 0.0752 &  0.0148 & T     \\
p527 & 22.5446 & 0.0839 & 22.3348 & 0.1173 & 53747.3342 & 2.3997 &  0.3779 & 1.7257 &  0.1832 & 0.0998 & -0.0266 & F    \\
p528 & 24.0024 & 0.0821 & 23.7831 & 0.1830 & 53734.2394 & 2.0274 &  4.2584 & 2.0348 &  0.1892 & 0.1422 &  0.1392 & F    \\
p534 & 23.3210 & 0.1333 & 23.4629 & 0.2933 & 53742.3189 & 7.0535 & -0.8193 & 3.4511 & -0.1615 & 0.1749 &  0.5612 & F    \\
q002 & 22.8550 & 0.1007 & 22.6752 & 0.0487 & 54001.9704 & 0.6189 & -2.6505 & 0.5734 &  0.1563 & 0.0982 &  0.0027 & T     \\
q006 & 22.8905 & 0.1105 & 22.7712 & 0.0432 & 53996.3154 & 1.0510 & -2.1751 & 0.5566 &  0.0963 & 0.0925 &  0.0054 & T     \\
q007 & 22.2260 & 0.0812 & 21.5884 & 0.0262 & 54000.7846 & 0.3328 &  0.2380 & 0.2772 &  0.6067 & 0.0634 &  0.0020 & F    \\
q008 & 21.7498 & 0.0559 & 21.6706 & 0.0225 & 54006.8207 & 0.2427 & -0.2647 & 0.1775 &  0.0552 & 0.0491 &  0.0003 & T     \\
q014 & 21.9967 & 0.0719 & 21.8155 & 0.0279 & 54008.3365 & 0.3058 &  0.9766 & 0.2655 &  0.1545 & 0.0601 &  0.0028 & T     \\
q022 & 21.8703 & 0.0806 & 21.6339 & 0.0289 & 53992.4503 & 1.0168 &  0.3006 & 0.3211 &  0.2095 & 0.0661 & -0.0013 & T     \\
q048 & 23.0639 & 0.0729 & 22.9408 & 0.0529 & 54023.6837 & 1.2934 & -2.2007 & 0.9229 &  0.1000 & 0.0834 & -0.0102 & T     \\
q049 & 22.7786 & 0.0759 & 22.7394 & 0.0592 & 54016.4163 & 0.4863 &  0.8448 & 0.5649 &  0.0150 & 0.0747 &  0.0049 & T     \\
q054 & 21.9276 & 0.0523 & 21.9448 & 0.0253 & 54025.3712 & 0.4783 &  0.6215 & 0.2964 & -0.0403 & 0.0500 &  0.0000 & T     \\
q061 & 23.2000 & 0.0767 & 22.7918 & 0.0303 & 54027.3989 & 0.9402 & -0.0799 & 0.5965 &  0.3796 & 0.0692 &  0.0037 & F    \\
q067 & 20.3989 & 0.0929 & 20.3907 & 0.0277 & 54034.7868 & 0.1961 &  0.8291 & 0.2075 & -0.0155 & 0.0740 &  0.0013 & T     \\
q069 & 22.0914 & 0.1004 & 21.8677 & 0.0477 & 54018.4893 & 0.7645 & -2.1882 & 0.3435 &  0.1992 & 0.0777 &  0.0008 & F    \\
q075 & 22.3419 & 0.0534 & 22.4547 & 0.0496 & 54018.8690 & 0.4026 &  0.6685 & 0.4024 & -0.1341 & 0.0673 &  0.0011 & T     \\
q102 & 22.6528 & 0.0432 & 22.6330 & 0.0377 & 54031.4251 & 0.4495 &  0.3796 & 0.3896 & -0.0038 & 0.0551 & -0.0019 & T     \\
q106 & 22.7735 & 0.0482 & 22.8680 & 0.0566 & 54037.0120 & 0.4339 &  0.2544 & 0.3763 & -0.1158 & 0.0701 &  0.0015 & T     \\
q107 & 23.6076 & 0.0633 & 23.6306 & 0.1206 & 54035.2369 & 0.8985 &  0.3444 & 0.6625 & -0.0458 & 0.1037 &  0.0097 & T     \\
q108 & 23.7523 & 0.0967 & 23.6387 & 0.1510 & 54017.0607 & 0.8552 & -0.8286 & 0.8402 &  0.0895 & 0.1431 &  0.0239 & T     \\
q112 & 23.5556 & 0.0780 & 23.4724 & 0.1251 & 54034.8121 & 1.6635 &  3.6606 & 1.2495 &  0.0558 & 0.1118 &  0.0448 & F    \\
q114 & 23.5407 & 0.0686 & 23.6445 & 0.1346 & 54039.8512 & 0.9367 & -0.8345 & 0.7933 & -0.1241 & 0.1061 &  0.0171 & T     \\
q125 & 22.4435 & 0.0775 & 22.4027 & 0.0402 & 54001.4395 & 1.6448 & -0.3898 & 0.4623 &  0.0175 & 0.0625 & -0.0040 & T     \\
r186 & 21.3735 & 0.0490 & 21.3828 & 0.0237 & 54045.4268 & 0.1922 &  0.4117 & 0.1644 & -0.0323 & 0.0460 & -0.0005 & T     \\
r190 & 22.3083 & 0.0514 & 22.2945 & 0.0294 & 54063.3751 & 0.3907 &  1.1219 & 0.2884 & -0.0103 & 0.0567 &  0.0008 & T     \\
r193 & 23.3562 & 0.0472 & 23.6080 & 0.0939 & 54052.6620 & 0.6757 &  1.0114 & 0.4539 & -0.2704 & 0.0858 &  0.0036 & F    \\
r195 & 23.3975 & 0.0615 & 23.2803 & 0.0771 & 54052.7438 & 0.6851 &  0.3250 & 0.5450 &  0.0921 & 0.0907 &  0.0049 & T     \\
r199 & 22.9096 & 0.0657 & 22.8114 & 0.0568 & 54042.5490 & 0.4736 &  0.1856 & 0.3997 &  0.0735 & 0.0717 & -0.0014 & T     \\
r200 & 22.5015 & 0.0877 & 22.0856 & 0.0307 & 54066.4317 & 0.5870 &  1.3868 & 0.5602 &  0.3859 & 0.0798 &  0.0210 & F    \\
r206 & 23.4720 & 0.0515 & 23.5624 & 0.1021 & 54055.0639 & 0.8126 & -0.4959 & 0.4651 & -0.1112 & 0.1015 &  0.0058 & T     \\
r207 & 23.2020 & 0.0696 & 23.1964 & 0.0814 & 54045.7051 & 0.5134 & -0.1189 & 0.4520 & -0.0173 & 0.0933 &  0.0104 & T     \\
r209 & 22.6669 & 0.0504 & 22.6848 & 0.0377 & 54052.0218 & 0.5171 & -0.3448 & 0.2762 & -0.0402 & 0.0584 &  0.0001 & T     \\
r212 & 23.7139 & 0.0651 & 23.8608 & 0.1366 & 54055.3079 & 1.0731 & -1.3401 & 0.5881 & -0.1660 & 0.1241 &  0.0105 & T     \\
r213 & 22.1991 & 0.0509 & 22.1173 & 0.0230 & 54063.5615 & 0.2399 & -0.0183 & 0.2188 &  0.0575 & 0.0478 &  0.0006 & T     \\
r225 & 23.7168 & 0.0913 & 23.3714 & 0.0751 & 54052.8641 & 1.6453 & -0.6543 & 0.7490 &  0.3180 & 0.1156 & -0.0358 & F    \\
r230 & 21.4134 & 0.0556 & 21.4469 & 0.0210 & 54071.4034 & 0.1394 &  0.0256 & 0.1645 & -0.0558 & 0.0462 &  0.0012 & T     \\
r311 & 24.0307 & 0.0969 & 23.8825 & 0.2108 & 54058.7940 & 2.3796 &  0.8043 & 1.3055 &  0.1222 & 0.1493 &  0.0328 & T     \\
r317 & 23.9761 & 0.1507 & 23.6856 & 0.0748 & 54061.7527 & 1.2865 &  0.4075 & 1.1008 &  0.2628 & 0.1418 &  0.0139 & F    \\
r318 & 20.7156 & 0.1004 & 20.5668 & 0.0343 & 54082.7021 & 0.4279 &  3.7147 & 0.5835 &  0.1202 & 0.0867 &  0.0059 & F    \\
r322 & 22.9680 & 0.0518 & 23.0576 & 0.0524 & 54077.7130 & 0.3442 &  0.3277 & 0.4020 & -0.1111 & 0.0641 &  0.0060 & T     \\
s340 & 23.2475 & 0.1171 & 23.1487 & 0.0945 & 54071.0726 & 0.6515 &  1.7077 & 0.8404 &  0.0728 & 0.1070 &  0.0407 & T     \\
s346 & 22.0831 & 0.0945 & 22.1017 & 0.0530 & 54077.7498 & 0.8850 &  0.4304 & 0.5864 & -0.0415 & 0.0707 &  0.0051 & F    \\
s347 & 21.9412 & 0.0745 & 21.8413 & 0.0355 & 54101.7341 & 0.4543 &  1.9025 & 0.5544 &  0.0737 & 0.0660 &  0.0114 & F    \\
s349 & 21.9374 & 0.0860 & 21.7752 & 0.0302 & 54085.4942 & 0.6436 & -1.4941 & 0.6750 &  0.1379 & 0.0737 &  0.0105 & T     \\
s350 & 23.8269 & 0.0525 & 23.8425 & 0.1088 & 54095.0873 & 1.0240 & -0.4534 & 0.8585 & -0.0378 & 0.0945 &  0.0242 & T     \\
s351 & 24.2855 & 0.0801 & 24.1537 & 0.1674 & 54088.6564 & 1.6628 &  0.2173 & 1.4625 &  0.1065 & 0.1310 &  0.0363 & T     \\
s353 & 23.8244 & 0.0821 & 23.4622 & 0.0996 & 54083.4828 & 1.2715 & -1.3897 & 0.9058 &  0.3352 & 0.1233 &  0.0463 & F    \\
s354 & 23.6884 & 0.0433 & 23.7003 & 0.0767 & 54091.4525 & 1.1957 &  1.0084 & 0.7540 & -0.0353 & 0.0828 &  0.0009 & T     \\
s355 & 23.9028 & 0.0490 & 23.9202 & 0.1033 & 54089.8178 & 1.1111 & -0.3781 & 0.8920 & -0.0396 & 0.0928 &  0.0203 & T     \\
s370 & 22.6954 & 0.0451 & 22.7677 & 0.0417 & 54096.8170 & 0.5367 &  0.7838 & 0.4880 & -0.0945 & 0.0590 &  0.0021 & T     \\
s372 & 24.0335 & 0.0686 & 24.2893 & 0.1424 & 54089.8789 & 1.2827 & -1.3515 & 1.1317 & -0.2727 & 0.1054 &  0.0283 & F    \\
s373 & 23.9640 & 0.0506 & 24.1761 & 0.1167 & 54090.4976 & 1.1778 & -0.1033 & 0.8617 & -0.2308 & 0.1020 &  0.0171 & T     \\
s374 & 24.1435 & 0.0676 & 24.0899 & 0.1608 & 54094.4964 & 1.6398 &  0.3000 & 1.2940 &  0.0295 & 0.1187 &  0.0603 & T     \\
s375 & 23.0683 & 0.0712 & 23.0140 & 0.0796 & 54103.4443 & 1.0471 &  1.9149 & 1.1050 &  0.0288 & 0.0728 &  0.0116 & T     \\
s377 & 22.4095 & 0.0529 & 22.2456 & 0.0359 & 54083.5998 & 1.0858 &  1.3617 & 0.6105 &  0.1371 & 0.0574 & -0.0052 & T     \\
s379 & 20.7474 & 0.0863 & 20.7618 & 0.0286 & 54102.6432 & 0.1802 &  0.2934 & 0.2928 & -0.0372 & 0.0646 &  0.0075 & T     \\
s380 & 23.8648 & 0.0752 & 23.5938 & 0.1271 & 54099.9126 & 0.9675 & -0.5541 & 0.9387 &  0.2444 & 0.1219 &  0.0329 & T     \\
x017 & 22.6885 & 0.0510 & 22.4829 & 0.0374 & 54379.5261 & 1.2391 & -0.4830 & 0.5868 &  0.1798 & 0.0681 & -0.0120 & F    \\
x020 & 23.9894 & 0.1303 & 24.1161 & 0.2289 & 54373.0684 & 1.4222 & -0.5980 & 1.3055 & -0.1467 & 0.1754 &  0.0890 & T     \\
x025 & 22.2673 & 0.0822 & 22.2316 & 0.0345 & 54357.8319 & 0.6157 & -0.6693 & 0.4700 &  0.0128 & 0.0727 &  0.0165 & T     \\
x028 & 23.4907 & 0.0799 & 23.4519 & 0.1104 & 54372.4066 & 1.0017 &  1.6558 & 0.9596 &  0.0139 & 0.1238 &  0.0519 & T     \\
x033 & 22.3561 & 0.0551 & 22.4182 & 0.0477 & 54389.4339 & 0.4386 &  0.5885 & 0.4297 & -0.0843 & 0.0606 & -0.0036 & T     \\
x034 & 23.3350 & 0.0705 & 23.1830 & 0.0685 & 54373.2170 & 0.5694 & -1.7059 & 0.4758 &  0.1280 & 0.0907 &  0.0060 & T     \\
x038 & 23.3872 & 0.0658 & 22.9736 & 0.0847 & 54386.8216 & 0.8979 &  3.6348 & 0.8110 &  0.3817 & 0.0942 & -0.0063 & F    \\
x039 & 22.8000 & 0.0458 & 22.9287 & 0.0991 & 54377.2993 & 0.6764 & -0.7227 & 0.4299 & -0.1486 & 0.0866 &  0.0138 & T     \\
x055 & 21.4731 & 0.0497 & 21.4423 & 0.0314 & 54371.7267 & 0.2240 & -1.0790 & 0.1778 &  0.0083 & 0.0531 & -0.0027 & F    \\
x066 & 21.7553 & 0.0530 & 21.8051 & 0.0274 & 54354.9573 & 0.6157 &  0.0524 & 0.3102 & -0.0718 & 0.0576 & -0.0027 & T     \\
x071 & 22.9287 & 0.0514 & 23.0307 & 0.0493 & 54394.9566 & 0.3462 &  0.4667 & 0.3329 & -0.1234 & 0.0650 &  0.0028 & T     \\
x077 & 23.0453 & 0.0380 & 23.0271 & 0.0588 & 54390.2104 & 0.5707 &  0.8043 & 0.3618 & -0.0056 & 0.0662 & -0.0031 & T     \\
x080 & 22.9853 & 0.0742 & 22.8054 & 0.0549 & 54385.9402 & 1.0200 & -0.1654 & 0.6365 &  0.1543 & 0.0931 & -0.0146 & T     \\
x085 & 23.6371 & 0.0608 & 23.7956 & 0.1542 & 54391.8397 & 0.7719 & -0.5811 & 0.5386 & -0.1779 & 0.1205 &  0.0037 & T     \\
x089 & 23.9825 & 0.0885 & 23.6363 & 0.1118 & 54388.3302 & 1.2429 &  1.0622 & 1.0014 &  0.3173 & 0.1224 & -0.0117 & F    \\
x093 & 24.0569 & 0.0682 & 23.8930 & 0.1565 & 54386.3484 & 1.1756 & -3.1692 & 1.1104 &  0.1411 & 0.1687 & -0.0512 & F    \\
x107 & 19.9776 & 0.1103 & 20.0055 & 0.0335 & 54404.9748 & 0.2586 &  1.3476 & 0.1648 & -0.0513 & 0.0863 & -0.0050 & T     \\
y125 & 21.8048 & 0.0486 & 21.7984 & 0.0215 & 54412.3552 & 0.4591 &  0.9537 & 0.2956 & -0.0173 & 0.0455 &  0.0002 & T     \\
y127 & 22.9975 & 0.0502 & 23.1558 & 0.0749 & 54406.4834 & 0.4584 &  0.5374 & 0.4629 & -0.1786 & 0.0801 &  0.0047 & T     \\
y134 & 22.0532 & 0.0588 & 22.0157 & 0.0241 & 54418.7132 & 0.4025 & -1.2900 & 0.5225 &  0.0151 & 0.0544 &  0.0060 & F    \\
y136 & 23.7734 & 0.0531 & 23.2402 & 0.0720 & 54413.2097 & 0.7646 &  1.8555 & 0.6512 &  0.5017 & 0.0869 & -0.0067 & F    \\
y137 & 22.1794 & 0.0444 & 22.1948 & 0.0286 & 54420.0259 & 0.2651 &  0.7089 & 0.2288 & -0.0386 & 0.0501 & -0.0018 & T     \\
y142 & 23.1411 & 0.0372 & 23.0899 & 0.0634 & 54422.5750 & 0.4331 &  0.6207 & 0.3211 &  0.0269 & 0.0689 &  0.0023 & T     \\
y143 & 22.8987 & 0.0480 & 22.9255 & 0.0437 & 54406.4119 & 0.5055 &  0.6174 & 0.3462 & -0.0496 & 0.0566 &  0.0013 & T     \\
y145 & 23.0351 & 0.0423 & 23.0817 & 0.0682 & 54420.7813 & 0.5852 &  1.7521 & 0.4795 & -0.0700 & 0.0738 &  0.0037 & T     \\
y151 & 23.3770 & 0.0599 & 23.3508 & 0.0805 & 54428.4959 & 0.4368 &  0.2279 & 0.4901 &  0.0027 & 0.0843 &  0.0089 & T     \\
y154 & 23.5828 & 0.0402 & 23.8149 & 0.0861 & 54418.9368 & 0.9335 &  0.3117 & 0.5900 & -0.2507 & 0.0783 &  0.0061 & F    \\
y158 & 23.0390 & 0.0428 & 23.0350 & 0.0419 & 54423.9295 & 0.3869 &  0.7066 & 0.3417 & -0.0195 & 0.0568 &  0.0025 & T     \\
y163 & 24.0333 & 0.0673 & 23.7489 & 0.1486 & 54421.9164 & 0.9259 & -1.2513 & 0.7018 &  0.2583 & 0.1334 &  0.0031 & F    \\
y175 & 22.8360 & 0.0601 & 22.6964 & 0.0459 & 54425.8623 & 0.2861 & -1.9635 & 0.3382 &  0.1161 & 0.0685 & -0.0007 & T     \\
y177 & 21.6761 & 0.0493 & 21.6179 & 0.0223 & 54437.7168 & 0.2485 &  1.1990 & 0.2590 &  0.0333 & 0.0456 &  0.0003 & T     \\
z180 & 22.5201 & 0.0375 & 22.5149 & 0.0276 & 54442.8254 & 0.3996 &  0.4254 & 0.2769 & -0.0181 & 0.0469 &  0.0006 & T     \\
z181 & 23.6384 & 0.0449 & 23.6948 & 0.0923 & 54439.2132 & 0.8229 & -0.1018 & 0.5110 & -0.0782 & 0.0908 &  0.0117 & T     \\
z183 & 21.4047 & 0.0502 & 21.4208 & 0.0207 & 54437.4468 & 0.2451 &  0.9457 & 0.1815 & -0.0395 & 0.0438 &  0.0001 & T     \\
z185 & 22.5041 & 0.0477 & 22.6490 & 0.0408 & 54431.6451 & 0.3612 & -0.0396 & 0.3277 & -0.1650 & 0.0566 & -0.0013 & T     \\
z187 & 21.7861 & 0.0520 & 21.7779 & 0.0205 & 54444.4417 & 0.3247 & -1.5587 & 0.3057 & -0.0136 & 0.0464 &  0.0017 & F    \\
z200 & 23.0644 & 0.0512 & 23.0241 & 0.0454 & 54453.2799 & 0.3546 & -0.0769 & 0.4278 &  0.0168 & 0.0606 &  0.0013 & T     \\
z202 & 20.7892 & 0.0644 & 20.8219 & 0.0211 & 54449.9709 & 0.1539 &  0.0645 & 0.1891 & -0.0551 & 0.0520 &  0.0021 & F    \\
z203 & 23.4393 & 0.1337 & 23.2272 & 0.0496 & 54452.9035 & 0.6130 &  2.0928 & 0.8403 &  0.1840 & 0.1075 &  0.0427 & F    \\
z204 & 23.5196 & 0.0648 & 23.5714 & 0.1171 & 54453.3551 & 0.7247 &  0.2490 & 0.7035 & -0.0740 & 0.0939 & -0.0006 & T     \\
z205 & 22.5140 & 0.0439 & 22.4191 & 0.0344 & 54453.8289 & 0.2631 &  0.7741 & 0.3069 &  0.0697 & 0.0513 & -0.0007 & T     \\
z208 & 23.1779 & 0.0733 & 23.2067 & 0.0664 & 54457.1693 & 0.8213 &  1.9027 & 1.0265 & -0.0527 & 0.0708 &  0.0222 & T     \\
\end{longtable}                                           

\tablenotetext{a}{SALT2 does not directly report distance estimates. The distance modulus is determined using a global fit for all \snia\ together with other cosmological parameters.}
\tablenotetext{b}{While the SALT2 shape estimates are strongly affected by measurements pre-maximum brightness, it uses significantly more low-S/N measurements on the decline, as well as measurements for faint and/or high-$z$ objects. Consequently, the cut on the number of measurements post-maximum has very little impact. We instead require that a total of 8 observations be used in the fit, to ensure that the measured parameters are reliable.}
\tablenotetext{c}{We use the updated SALT2 color law described by \citet{guy10}. This differs significantly from the CCM89 law in the near-UV.}
\tablenotetext{d}{Covariances between all the fit parameters --- Cov($m_{B}$,$x_{1}$), Cov($m_{B}$,$c$), and Cov($x_{1}$,$c$) --- are calculated, and these values will be included in the machine-readable tables provided with this work.}
\tablenotetext{e}{Flag describing if the object passes (T) or fails (F) the light-curve quality cuts for SALT described by WV07 and the shape and color cuts described by \citet{conley11}.}

\end{center}
\end{landscape}
\onehalfspacing

